Stabilising priors for robust Bayesian deep learning

Bayesian neural networks (BNNs) have developed into useful tools for probabilistic modelling due to recent advances in variational inference enabling large scale BNNs. However, BNNs remain brittle and hard to train, especially: (1) when using deep architectures consisting of many hidden layers and (2) in situations with large weight variances. We use signal propagation theory to quantify these challenges and propose self-stabilising priors. This is achieved by a reformulation of the ELBO to allow the prior to influence network signal propagation. Then, we develop a stabilising prior, where the distributional parameters of the prior are adjusted before each forward pass to ensure stability of the propagating signal. This stabilised signal propagation leads to improved convergence and robustness making it possible to train deeper networks and in more noisy settings.

==> adElbo.tex <==
\section{Bayesian inference in deep neural networks}

Given a set of observations $\mathcal{D} = \{(\mathbf{x}_n, \mathbf{y}_n), n = 1, ..., N\}$, we use a Bayesian approach to model the distribution over an outcome $\mathbf{y}$ conditioned on an input $\mathbf{x}$, i.e. $p(\mathbf{y}| \mathbf{x})$, using a parametrised function of the input $f(\mathbf{x}; \theta)$ with parameters $\theta$. 
We choose our input-output function map to be a fully-connected feedforward neural network. 
Specifically, given an input $\mathbf{x}^0 \in \mathbb{R}^{D_0}$, such a deep neural network can be recursively defined by 
\begin{align}
	 \mathbf{h}^l = W^l\mathbf{x}^{l} + \mathbf{b}^l \textcolor{white}{white} \mathbf{x}^{l} = g(\mathbf{h}^{l-1}), \textcolor{white}{spa} \text{ for } l = 1, ..., L
	\label{eq: noisy deep model}
\end{align}
where the weights $W^l \in \mathbb{R}^{D_l \times D_{l-1}}$ and the biases $\mathbf{b}^l \in \mathbb{R}^{D_l}$ constitute the model parameters $\theta = \{W^l, \mathbf{b}^l\}^L_1$. We denote the dimensionality of the hidden layers using $D_l$ and compute activations at each layer element-wise using an activation function $g(\cdot)$.
% with weights $W^l \in \mathbb{R}^{D_l \times D_{l-1}}$ and biases $\mathbf{b}^l \in \mathbb{R}^{D_l}$, 


To incorporate our prior belief concerning the model parameters, we specify a prior distribution $p_\alpha(W)$ over the weights described by parameters $\alpha$, while treating the biases as being deterministic. 
This initial belief is updated using observed samples together with Bayes rule to obtain a posterior distribution $p(W|\mathcal{D}) = p(\mathcal{D}|W)p_\alpha(W)/\int p(\mathcal{D}|W)dW$. 
Unfortunately, for deep neural networks, a simple application of Bayes rule is computationally intractable because it requires an extremely high-dimensional marginalisation over the weights. 
Instead, BNNs make use of variational inference.

\subsection{Variational inference}

Variational inference approaches estimation of the posterior as an optimisation problem. We use gradient based procedures to optimise for parameters $\phi$, of an approximating posterior distribution $q_\phi(W)$ in a family of potential approximate posteriors.  
The objective is to minimise the Kullback-Leibler (KL) divergence $\textrm{KL}(q_\phi(W)||p(W|\mathcal{D}))$ between $q_\phi(W)$ and the true posterior by maximising the \textit{evidence lower bound} (ELBO)  
\begin{align}
    \mathcal{L}_q & = L_\mathcal{D}(\phi, \theta) - \textrm{KL}(q_\phi(W)||p_\alpha(W)) \label{eq: elbo} \\ 
     L_\mathcal{D}(\phi, \theta) &= \sum^N_{n=1}\mathbb{E}_{q_\phi(W)}[\log p(\mathbf{y}_n| \mathbf{x}_n, \theta)]. \nonumber
\end{align}
The first term in \eqref{eq: elbo} is the expected log-likelihood of the data under $q_{\phi}(W)$ and the second term is the KL divergence between the approximate posterior and the prior over the weights, which acts as a regulariser. 

\subsection{Stochastic backpropagation}

The expectations in \eqref{eq: elbo} can be estimated efficiently using the reparametrisation trick in stochastic backpropagation \citep{kingma2013auto, rezende2014stochastic}. Instead of sampling directly from the approximating posterior, samples $\epsilon$ are taken from an auxiliary distribution $p(\epsilon)$, which does not depend on any parameters, and transformed using a function $\xi$ that is differentiable in the parameters $\phi$, such that  $W = \xi(\epsilon, \phi)$. This technique gives an unbiased Monte Carlo estimator of the log-likelihood for a specific mini-batch of size $M$ as
\begin{align}
    \label{eq: monte carlo estimator}
    L_\mathcal{D}(\phi, \theta) & \approx \frac{N}{M}\sum^M_{m=1} \log p(\mathbf{y}_m|\mathbf{x}_m, \mathbf{b}, W = \xi(\epsilon, \phi)) \\
    \nabla_\phi L_\mathcal{D}(\phi, \theta) & \approx \frac{N}{M}\sum^M_{m=1} \nabla_\phi \log p(\mathbf{y}_m|\mathbf{x}_m, \mathbf{b}, W = \xi(\epsilon, \phi)).
\end{align}
where we can take derivative directly w.r.t. the variational parameters $\phi$.
We optimise the ELBO $\mathcal{L}_q$ using stochastic gradient ascent. 


%Note that $\tilde{q}$ and $q$ share the same parameters. Also, the second term in the above equation is the cross entropy between the product mixture of the current posterior and prior $pq$ with the current posterior $q$ which we write as $\textrm{H}[ \tilde{q}, q]$. 

% Reparameterisation of the sampled weights give
% \begin{align}
%     \label{eq: adelbo reparam}
%     \log p(\mathbf{y} | \mathbf{x}) & \geq \mathbb{E}_{p(\epsilon)} \left [  \log p(\mathbf{y}|\mathbf{x}, W = f(\epsilon, \phi)) \right] +  \textrm{H}[ \tilde{q}, q]\\ 
%     & = \mathcal{L}_{\tilde{q}, \textrm{H}}
% \end{align}


% Often for prediction, the mean of the above conditional is modeled using a parameterised function, such that $\mathbb{E}[p(\mathbf{y}| \mathbf{x})] = f(\mathbf{x}, W)$ and  the parameters (weights) $W$ are optimised using maximum likelihood estimation (MLE). However, MLE can suffer severely from overfitting. Furthermore, by being a point estimator, MLE does not provide a full conditional distribution and therefore cannot provide any estimates of uncertainty, or perform model averaging. 

==> relatedWork.tex <==
\section{Related work}

Scaling BNNs has only recently become feasible with stochastic variational methods \citep{graves2011practical, blundell2015weight,rezende2014stochastic,hoffman2013stochastic}, making it possible to train deep Bayesian models. Despite these advances, high variance remains an issue. Therefore, it is standard practice to use various variance reduction techniques and tricks to get variational inference to work at scale \citep{lrt, zhang2018advances}.

%\cite{graves2011practical, blundell2015weight, hoffman2013stochastic ,rezende2014stochastic}

This work builds on \citep{pretorius2018critical}, which extended the analysis of signal propagation in \citep{poole2016exponential, schoenholz2016deep} for deterministic ReLU networks with stochastic regularisation. 
In light of recent links between stochastic regularisation techniques and variational inference \citep{gal2016dropout, lrt}, we relate the initialisation techniques derived in \cite{pretorius2018critical}, to an iteratively updating prior to stabilise the flow of information through ReLU networks throughout training.


Priors for BNNs have been designed for many applications such as automatic relevance determination \citep{neal2012bayesian}, compression \citep{louizos2017bayesian}, sparsification \citep{molchanov2017variational, carvalho2009handling, ghosh2018structured} and reliable uncertainty estimation \citep{hafner2019reliable}. Our prior is designed for robust learning, related to \cite{Wu}, which calculate deterministic approximations to the moments propagating through the network by also making use of the central limit theorem. A key difference is that we formulate a new prior and build on a large body of work in Monte Carlo variational inference techniques. Another interesting connection with our work is variance networks \citep{neklyudov2018variance}, which have the required conditions for stable signal propagation. However, we find it impossible to train variance networks of any meaningful depth.

